CoTEVer: Chain of Thought Prompting Annotation Toolkit for Explanation Verification

Chain-of-thought (CoT) prompting enables large language models (LLMs) to solve complex reasoning tasks by generating an explanation before the final prediction. Despite it's promising ability, a critical downside of CoT prompting is that the performance is greatly affected by the factuality of the generated explanation. To improve the correctness of the explanations, fine-tuning language models with explanation data is needed. However, there exists only a few datasets that can be used for such approaches, and no data collection tool for building them. Thus, we introduce CoTEVer, a tool-kit for annotating the factual correctness of generated explanations and collecting revision data of wrong explanations. Furthermore, we suggest several use cases where the data collected with CoTEVer can be utilized for enhancing the faithfulness of explanations. Our toolkit is publicly available at https://github.com/SeungoneKim/CoTEVer.

==> table/csqaprompt.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}

\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabularx}{500pt}{l}
%\begin{longtable}{p{1.0\textwidth}} 
\midrule \\
Prompt for Multiple Choice Questions \\
 \midrule 
Question : What do people use to absorb extra ink from a fountain pen?\\
Options : shirt pocket, calligrapher’s hand, inkwell, desk drawer, blotter\\
\\
Q\#1 : What is a shirt pocket?\\
A\#1 : A shirt pocket is a small bag attached to a shirt used to carry things in.\\
Q\#2 : What is a calligrapher's hand?\\
A\#2 : A calligrapher's hand is a hand of a person who is skilled at the art of producing beautiful writing,\\
\quad\quad\quad often with a special pen or brush.\\
Q\#3 : What is a inkwell?\\
A\#3 : A inkwell is a container for ink.\\
Q\#4 : What is a desk drawer?\\
A\#4 : A desk drawer is a box-shaped container, that is used for keeping things in.\\
Q\#5 : What is a blotter?\\
A\#5 : A blotter is a large piece of paper that is used to absorb ink.\\
Q\#6 : What do people use to absorb extra ink from a fountain pen?\\
A\#6 : The answer must be an item that can absorb ink. \\
\quad\quad\quad Of the above choices, blotter is made to absorb ink.\\
So, the answer is blotter.\\
\\
Q : What home entertainment equipment requires cable?\\
Options : radio shack, substation, television, cabinet\\
\\
Q\#1 : What is a radio shack?\\
A\#1 : Radio shack is an American retailer that sells consumer electronics.\\
Q\#2 : What is a substation?\\
A\#2 : Substation is a place that allows electricity to go from one part of the electricity production \\
\quad\quad\quad system to another.\\
Q\#3 : What is a television?\\
A\#3 : Television is a device that receives electrical signals from a cable and changes them into \\
\quad\quad\quad moving images or sound.\\
Q\#4 : What is a cabinet?\\
A\#4 : Cabinet is a piece of furniture with shelves, cupboards, or drawers, used for storing or \\
\quad\quad\quad showing things.\\
Q\#5 : What home entertainment equipment requires cable?\\
A\#5 : The answer must be an entertainment equipment and also require cable.\\ 
\quad\quad\quad Of the above choices, television is a entertainment equipment and also requires cable to receive electrical signals.\\
So the answer is television.\\
\\
Question : The fox walked from the city into the forest, what was it looking for?\\
Options : pretty flower, shen house, natural habitat, storybook \\
\\
Q\#1 : What are flowers?\\
A\#1 : A flower is the part of a plant which is often brightly coloured, grows at the end of a stem.\\
Q\#2 : What is a hen house?\\
A\#2 : A hen house is a house made to keep chickens inside.\\
Q\#3 : What is natural habitat?\\
A\#3 : Natural habitat is an environment in which animals and plants grow.\\
Q\#4 : What is a story book?\\
A\#4 : Story book is a book of stories for children.\\
Q\#5 : The fox walked from the city into the forest, what was it looking for?\\
A\#5 : The answer must be something in the forest. \\
\quad\quad\quad Of the above choices, a fox might look for natural habitat to live in that is in the forest.\\
So the answer is natural habitat.\\
\\
Question : Sammy wanted to go to where the people were. Where might he go?\\
Options : populated areas, race track, desert, apartment, roadblock \\
Q\#1 : What is a populated area?\\
A\#1 : A populated area is a place were a lot of people are.\\
Q\#2 : What is a race track?\\
A\#2 : A race track is a track on which horses or race cars race on.\\
Q\#3 : What is a desert?\\
A\#3 : A desert is a large area of land, usually in a hot region, where there is almost no water, rain, trees, plants, or people.\\
Q\#4 : What is an apartment?\\
A\#4 : An apartment is a set of rooms for living in.\\
Q\#5 : What is a roadblock?\\
A\#5 : A roadblock is a barrier set up across a road for halting or hindering traffic.\\
Q\#6 : Sammy wanted to go to where the people were. Where might he go?\\
A\#6 : The answer must be a place with a lot of people.
\quad\quad\quad Of the above choices, populated areas have a lot of people.\\
So the answer is populated areas.\\
\\
Question : Where do you put your grapes just before checking out?\\
Options : mouth, grocery cart, super market, fruit basket, fruit market\\
\\
Q\#1 : What is a mouth?\\
A\#1 : A mouth is the opening in the face of a person or animal.\\
Q\#2 : What is a grocery cart?\\
A\#2 : A grocery cart is a small vehicle that one would push to transport large or heavy objects while shopping.\\
Q\#3 : What is a super market?\\
A\#3 : A super market is a large shop which sells most types of food and other goods needed in home.\\
Q\#4 : What is a fruit basket?\\
A\#4 : A fruit basket is a light container used for storing fruits inside.\\
Q\#5 : What is a fruit market?\\
A\#5 : A fruit market is a place where people would sell fruits to customers.\\
Q\#6 : Where do you put your grapes just before checking out?\\
A\#6 : The answer should be the place where grocery items are placed before checking out. \\
\quad\quad\quad Of the above choices, grocery cart are used to hold grocery items conventionally before checking out.\\
So, the answer is grocery cart.\\
\\
Question : Google Maps and other highway and street GPS services have replaced what?\\
Options : united states, mexico, countryside, atlas \\
\\
Q\#1 : What is united states?\\
A\#1 : United States is a country or nation consisting of 50 states.\\
Q\#2 : What is mexico?\\
A\#2 : Mexico is a country in southern North America.\\
Q\#3 : What is a countryside?\\
A\#3 : A countryside is land not in towns, cities, or industrial areas, that is either used for farming or left in its natural condition.\\
Q\#4 : What is an atlas?\\
A\#4 : An atlas is a book of containing maps.\\
Q\#5 : Google Maps and other highway and street GPS services have replaced what?\\
A\#5 : The answer must be something that used to do what Google Maps and GPS services do, which is to give directions.\\ 
Of the above choices, only atlases are used to give directions.\\
So, the answer is atlas.\\
\\
Question : Before getting a divorce, what did the wife feel who was doing all the work?\\
Options : harder, anguish, bitterness, tears, sadness \\
\\
Q\#1 : What is the emotion of being harder?\\
A\#1 : Feeling harder means to feel angry about something.\\
Q\#2 : What is the emotion of being anguish?\\
A\#2 : Feeling anguish means to feel great mental suffering or physical pain.\\
Q\#3 : What is the emotion of being bitterness?\\
A\#3 : Feeling bitterness means to feel disappointing after being treated unfairly.\\
Q\#4 : What is the emotion of tears?\\
A\#4 : Feeling tears means to cry due to sad feelings.\\
Q\#5 : What is the emotion of sadness?\\
A\#6 : Feeling sad means to feel unhappy usually because something has happened that you do not like.\\
A\#6 : The answer should be the feeling of someone getting divorced who was doing all the work. \\
\quad\quad\quad Of the above choices, the wife should feel disappointing about the fact that she did all the work by herself.\\
So, the answer is bitterness.\\
\midrule 

\end{tabularx}%
}
\caption{Revising \citet{wei2022chain}'s CommonsenseQA prompt into a \citet{press2022measuring} style prompt}
\end{table*}
%\end{longtable}

==> table/sqaprompt.tex <==
\begin{table}[p]
\begin{tabular}{l}
{[}Example 1{]}                                                                                                                       \\
Question : Do hamsters provide food for   any animals?                                                                                \\
                                                                                                                                      \\
Q\#1 : What type of animals are hamsters?                                                                                             \\
A\#1 : Hamsters are prey animals.                                                                                                     \\
Q\#2 : Can prey animals be food for other   animals?                                                                                  \\
A\#2 : Prey are food for predators.                                                                                                   \\
Q\#3 : Do hamsters provide food for any   animals?                                                                                    \\
\begin{tabular}[c]{@{}l@{}}A\#3 :   Since hamsters are prey animals, and prey are food\\       for predetors, hamsters provide food   for some animals.\end{tabular} \\
So the answer is yes.                                                                                                                 \\
                                                                                                                                      \\
{[}Example 2{]}                                                                                                                       \\
Question : Could Brooke Shields succeed   at University of Pennsylvania?                                                              \\
                                                                                                                                      \\
Q\#1 : What university did Brooke Shields   went to?                                                                                  \\
A\#1 : Brooke Shields went to Princeton   University.                                                                                 \\
Q\#2 : Did Brooke Shields succeed at   Princeton University?                                                                          \\
\begin{tabular}[c]{@{}l@{}}A\#2 :   At Princeton University, she got all As and Bs while pursing her\\      bachelor's degree in French literature, meaning she had a successful\\      school life.\end{tabular} \\
\begin{tabular}[c]{@{}l@{}}Q\#3 :   How rigorous is Princeton University compared to University \\      of Pennsylvania?\end{tabular} \\
\begin{tabular}[c]{@{}l@{}}A\#3 :   Princeton University is about as academically rigorous as the\\      University of Pennsylvania because they have a similar ranking \\      according to U.S. News Rankings.\end{tabular} \\
Q\#4 : Could Brooke Shields succeed at   University of Pennsylvania?                                                                  \\
\begin{tabular}[c]{@{}l@{}}A\#4 :   Since University of Pennsylvania and University of Princeton\\       are in similar circumstances, Brooke   Shields has been successful\\       in University of Princeton, Brooke   Shields could also succeed at\\       the University of Pennsylvania.\end{tabular} \\
So the answer is yes.                                                                                                                 \\
                                                                                                                                      \\
{[}Example 3{]}                                                                                                                       \\
\begin{tabular}[c]{@{}l@{}}Question   : Hydrogen’s atomic number squared exceeds number \\      of Spice Girls?\end{tabular}          \\
                                                                                                                                      \\
Q\#1 : What is the atomic number of   Hydrogen?                                                                                       \\
A\#1 : Hydrogen has an atomic number of 1.                                                                                            \\
Q\#2 : What is 1 squared?                                                                                                             \\
A\#2 : 1 squared is 1.                                                                                                                \\
Q\#3 : How much Spice Girls are there?                                                                                                \\
A\#3 : There are 5 Spice Girls.                                                                                                       \\
Q\#4 : Hydrogen’s atomic number squared   exceeds number of Spice Girls?                                                              \\
\begin{tabular}[c]{@{}l@{}}A\#4 :   Since Hydrogen's atomic number squared is 1, the number of Spice \\      Girls are 5, and 1 is smaller than 5, Hydrogen’s atomic number squared   is\\       less than the number of Spice Girls.\end{tabular} \\
So the answer is no.                         
\end{tabular}
\end{table}


==> table/sqaprompt2.tex <==
\begin{table}[p]
\begin{tabular}{l}
{[}Example 4{]}                                                                  \\
Question : Is it common to see frost   during some college commencements?        \\
                                                                                 \\
Q\#1 : When does College commencement   ceremonies usually happen?               \\
\begin{tabular}[c]{@{}l@{}}A\#1 :   College commencement ceremonies can happen in December,\\      May, and June.\end{tabular} \\
Q\#2 : Does it usually frost in December?                                        \\
A\#2 : December is in the winter, so there   can be frost.                       \\
Q\#3 : Is it common to see frost during   some college commencements?            \\
\begin{tabular}[c]{@{}l@{}}A\#3 :   Since there can be frost in December and a college commencement \\      are held in December, there could be frost at some commencements.\end{tabular} \\
So the answer is yes.                                                            \\
                                                                                 \\
{[}Example 5{]}                                                                  \\
Question : Could a llama birth twice   during War in Vietnam (1945-46)?          \\
                                                                                 \\
Q\#1 : How long was the Vietnam war?                                             \\
A\#1 : The War in Vietnam was 6 months.                                          \\
Q\#2 : How long is the gestation period?                                         \\
A\#2 : The gestation period for a llama is   11 months.                          \\
Q\#3 : How long does it take for a llama   to birth twice?                       \\
\begin{tabular}[c]{@{}l@{}}A\#3 :   Since the gestation period for a llama is 11 months, and 11 times\\       2 is 22, it will take 22 months.\end{tabular} \\
Q\#4 : Could a llama birth twice during   War in Vietnam (1945-46)?              \\
\begin{tabular}[c]{@{}l@{}}A\#4 :   Since it takes 22 months for a llama to birth twice, War in Vietnam\\       was 6 months, and 22 is bigger than   6, llama could not give birth twice\\       during the War in Vietnam.\end{tabular} \\
So the answer is no.                                                             \\
                                                                                 \\
{[}Example 6{]}                                                                  \\
Question :  Would a pear sink in water?                                          \\
                                                                                 \\
Q\#1 : What is the density of a pear?                                            \\
A\#1 : The density of a pear is about   0.6g/cm3.                                \\
Q\#2 : What is the density of water?                                             \\
A\#2 : The density of water is 1g/cm3.                                           \\
Q\#3 : Is the density of pear smaller than   water?                              \\
A\#3 : Since 0.6 is smaller than 1, the   density of pear is smaller than water. \\
Q\#4 : If the density of an object is less   than water, what happens?           \\
A\#4 : Objects less dense than water   float.                                    \\
Q\#5 : Would a pear sink in water?                                               \\
A\#5 : Since a pear has a smaller density   than water, a pear would float.      \\
So the answer is no.                                                            
\end{tabular}
\end{table}

==> table/tmptable.tex <==
\begin{document}

\begin{table*}[tbp]
\newcommand\HH{\hspace{0pt}}
\NewTableCommand{\Mdois}{\SetCell[c=2]{preto=\justifying,wd=0.7\textwidth+2\tabcolsep}}
\NewTableCommand{\Mtres}{\SetCell[c=3]{preto=\justifying,wd=0.8\textwidth+4\tabcolsep}}
\SetTblrInner{rowsep=1pt}
\small
\centering
\caption{Especificação das Métricas do CVSS}
\label{tab:metricas-cvss}
\begin{tblr}{colspec={ m{0.1\textwidth} m{0.1\textwidth} m{0.1\textwidth} Q[preto=\justifying,wd={0.6\textwidth}] },colsep=\tabcolsep,cells={c,m}}
\toprule
\SetCell[r=11]{c}{\textbf{Métricas de Base}}   & \Mtres {Todas as métricas que servem de base para o cálculo da vulnerabilidade, de forma preliminar.}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ \cline{2-4} 
                                     & \SetCell[r=5]{c}{\textbf{Métricas de Explorabilidade}} & \Mdois {As métricas de explorabilidade refletem valores relativos ao componente afetado, bem como propriedades de uma vulnerabilidade que leve a cabo um ataque bem-sucedido.}                                &                                                                                                                                                                                                                                      \\ \cline{3-4} 
                                     &                                              & \SetCell[r=1]{c,m}\textbf{Vetor de Ataque (AV)}         & \SetCell[r=1]{c,m}
Contexto pela qual a exploração da vulnerabilidade é possível - o valor será tanto maior quanto mais um atacante conseguir atingir (lógica e fisicamente) para explorar o componente vulnerável.                                                                                                                                                                                                                                \\ \cline{3-4} 
                                     &                                              & \HH\textbf{Complexidade do Ataque (AC)}  & Condições para além do controlo do atacante que devem existir para explorar a vulnerabilidade.                                                                                                                                                                                                                                                                                                                                  \\ \cline{3-4} 
                                     &                                              & \textbf{Privilégios Necessários (PR)} & Nível de privilégios que um atacante deve possuir antes de explorar a vulnerabilidade com sucesso – quantos menos privilégios forem necessários, mais alta será a pontuação.                                                                                                                                                                                                                                                    \\ \cline{3-4} 
                                     &                                              & \textbf{Interação do Utilizador (UI)} & Captura a necessidade de um utilizador humano, diferente do atacante, participar no comprometimento bem-sucedido do componente vulnerável                                                                                                                                                                                                                                                                                       \\ \cline{2-4} 
                                     & \textbf{Contexto (S)}                                 & \Mdois {Captura se uma vulnerabilidade num componente vulnerável afeta os recursos noutros componentes para além do seu contexto de segurança.}                                                                                                                                                                                                                                                                                                     \\ \cline{2-4} 
                                     & \SetCell[r=4]{c}{\textbf{Métricas de Impacto}}         & \Mdois {Capturam os efeitos de uma vulnerabilidade explorada com sucesso no componente que sofre o pior resultado que está mais direta e previsivelmente associado ao ataque.}                                                                                                                                                                                                                                                                      \\ \cline{3-4} 
                                     &                                              & \HH\textbf{Confidencialidade (C)}        & Mede o impacto sobre a confidencialidade dos recursos de informação geridos por um componente de software graças a uma vulnerabilidade explorada com sucesso – a classificação é maior quando a perda para o componente afetado é maior.                                                                                                                                                                                        \\ \cline{3-4} 
                                     &                                              & \textbf{Integridade (I)}              & Mede o impacto na integridade de uma vulnerabilidade explorada com sucesso – a classificação é maior quando a consequência para o componente afetado é maior.                                                                                                                                                                                                                                                                   \\ \cline{3-4} 
                                     &                                              & \HH\textbf{Disponibilidade (A)}          & Mede o impacto na disponibilidade do componente afetado resultante de uma vulnerabilidade explorada com sucesso. Como a disponibilidade se refere à acessibilidade dos recursos de informação, os ataques que consomem largura de banda da rede, ciclos do processador ou espaço em disco impactam a disponibilidade do componente afetado – a classificação é maior quando a consequência para o componente impactado é maior. \\ \hline
\SetCell[r=4]{c}{\textbf{Métricas Temporais}}  & \Mtres {As métricas temporais medem o estado atual das técnicas de exploração ou disponibilidade de código, a existência de \textit{patches} ou uma solução de recurso (comumente designado em inglês por \textit{workaround}), ou a certeza da descrição da vulnerabilidade}                                                                                                                                                                                                                                        \\ \cline{2-4} 
                                     & \textbf{Exploração da Maturidade do Código (E)}       & \Mdois {Mede a probabilidade de a vulnerabilidade ser atacada e é normalmente baseada no estado atual das técnicas de exploração, disponibilidade de código de exploração ou exploração ativa \textit{in-the-wild}.}                                                                                                                                                                                                                                         \\ \cline{2-4} 
                                     & \textbf{Nível de Remediação (RL)}                     & \Mdois {É um fator importante para a priorização - quanto menos oficial EXPLICAR O QUE É OFICIAL?! e permanente for uma correção, maior será a pontuação de uma vulnerabilidade.}                                                                                                                                                                                                                                                                   \\ \cline{2-4} 
                                     & \textbf{Confiança no Reporte (RC)}                    & \Mdois {Mede o grau de confiança na existência da vulnerabilidade e na credibilidade dos detalhes técnicos conhecidos - quanto mais uma vulnerabilidade é validada pelo fornecedor ou outras fontes confiáveis, maior será a pontuação.}                                                                                                                                                                                                            \\ \hline
\SetCell[r=3]{c}{\textbf{Métricas Ambientais}} & \Mtres {As métricas ambientais permitem a personalização da pontuação do CVSS, dependendo da importância do ativo de TI afetado para a organização de um utilizador, medida em termos de controlos de segurança complementares e/ou alternativos implementados, confidencialidade, integridade e disponibilidade.}                                                                                                                                                                                 \\ \cline{2-4}
                                     & \textbf{Requisitos de Segurança (CR, IR, AR)}         & \Mdois {Permitem que o analista personalize a pontuação CVSS, dependendo da importância do ativo de TI afetado para a organização de um utilizador, medida em termos de confidencialidade, integridade ou disponibilidade - cada requisito de segurança tem três valores possíveis: Baixo, Médio ou Alto.}                                                                                                                                          \\ \cline{2-4}
                                     & \textbf{Métricas de Base Modificadas}                 & \Mdois {Permitem que o analista substitua as métricas básicas individuais com base em características específicas do ambiente de um utilizador; delas fazem parte a Modified Attack Vector (MAV), Modified Attack Complexity (MAC), Modified Privileges Required (MPR), Modified User Interaction (MUI), Modified Scope (MS), Modified Confidentiality (MC), Modified Integrity (MI) ou Modified Availability (MA).}                                \\
\bottomrule
\end{tblr}
\end{table*}

\end{document}
